A natural boundary of dark matter haloes revealed around the minimum bias and maximum infall locations

We explore the boundary of dark matter haloes through their bias and velocity profiles. Using cosmological $N$-body simulations, we show that the bias profile exhibits a ubiquitous trough that can be interpreted as created by halo accretion that depletes material around the boundary. The inner edge of the active depletion region is marked by the location of the maximum mass inflow rate that separates a growing halo from the draining environment. This inner depletion radius can also be interpreted as the radius enclosing a highly complete population of splashback orbits, and matches the optimal exclusion radius in a halo model of the large-scale structure. The minimum of the bias trough defines a characteristic depletion radius, which is located within the infall region bounded by the inner depletion radius and the turnaround radius, while approaching the turnaround radius in low mass haloes that have stopped mass accretion. The characteristic depletion radius depends the most on halo mass and environment. It is approximately $2.5$ times the virial radius and encloses an average density of $\sim 40$ times the background density of the universe, independent on halo mass but dependent on other halo properties. The inner depletion radius is smaller by $10-20\%$ and encloses an average density of $\sim 63$ times the background density. These radii open a new window for studying the properties of haloes.

==> Makefile <==
MAIN=main
OLD=old/main
BIB=ref.bib
STYLE=mnras.cls mnras.bst
#STYLE=mn2e_new.bst mn2e-bst.sty mn2e.cls aas_macros.sty mymn.bst
#timestr=`date +%a-%d-%b`
timestr=`date -Idate`
#lineno.sty
TC=pdflatex
#TC=latex

ifeq ($(TC), latex)
PC=dvipdf
else
PC=echo
endif

paper:
	$(TC) $(MAIN)
	bibtex $(MAIN)
	$(TC) $(MAIN)
	$(TC) $(MAIN)
	$(PC) $(MAIN)

diff:
	latexdiff $(OLD).tex $(MAIN).tex >diff.tex
	@make paper -e MAIN=diff
	@make clean -e MAIN=diff
	
tar: clean paper 
	mkdir tmp
	mkdir tmp/Figures
	cp $(MAIN).tex $(BIB) $(STYLE) Makefile tmp/
	cp Figures/* tmp/Figures/
	cd tmp;	tar -czhf $(MAIN).$(timestr).tar.gz *; mv $(MAIN).$(timestr).tar.gz ../
	
clean:
	\rm -rf tmp
	\rm -f $(MAIN).aux $(MAIN).log $(MAIN).toc $(MAIN).blg $(MAIN).dvi $(MAIN).ps $(MAIN).out $(MAIN).bbl
	\rm -f diff.aux diff.log diff.toc diff.blg diff.dvi diff.ps diff.out diff.bbl

ultclean:
	\rm -rf tmp
	\rm -f *.aux *.log *.toc *.blg *.dvi *.ps *.out *.bbl *.backup $(MAIN).*.tar.gz $(MAIN).pdf
	\rm -f diff.pdf diff.tex

